Hierarchical Variational Auto-Encoding for Unsupervised Domain Generalization

We address the task of domain generalization, where the goal is to train a predictive model such that it is able to generalize to a new, previously unseen domain. We choose a hierarchical generative approach within the framework of variational autoencoders and propose a domain-unsupervised algorithm that is able to generalize to new domains without domain supervision. We show that our method is able to learn representations that disentangle domain-specific information from class-label specific information even in complex settings where domain structure is not observed during training. Our interpretable method outperforms previously proposed generative algorithms for domain generalization as well as other non-generative state-of-the-art approaches in several hierarchical domain settings including sequential overlapped near continuous domain shift. It also achieves competitive performance on the standard domain generalization benchmark dataset PACS compared to state-of-the-art approaches which rely on observing domain-specific information during training, as well as another domain unsupervised method. Additionally, we proposed model selection purely based on Evidence Lower Bound (ELBO) and also proposed weak domain supervision where implicit domain information can be added into the algorithm.

==> app.tex <==
\appendix
\section{Pre-requisite}\label{sec:pre-requisite}
\paragraph{RKHS}
$RKHS(\mathcal{X}, k)$: for $x\in \mathcal{X}$, with kernel $k$, for $k(x, \cdot), f(\cdot) \in RKHS$\\
\begin{itemize}
\item $\langle k(x,\cdot), f(\cdot)\rangle = f(x)$
\item $\langle k(x,\cdot), k(x^{'},\cdot)\rangle$
 \end{itemize}
 with feature map $\phi(x)$,  $f(x) = \langle w, \phi(x)\rangle$, where $w$ is the coordinate of $f(\cdot)$ in RKHS. 

\paragraph{Riesz–Fréchet representation theorem} 
Let H  be a Hilbert space and $\varphi \in H^{*}$ where $H^{*}$ is the dual space of $H$(space of all linear functions on $H$). Then there exists $f\in H$ such that for any $\phi(x)\in H$, $\varphi (\phi(x))=\langle f,\phi(x)\rangle$. Moreover $\|f\|_{H}=\|\varphi \|_{H*}$. i.e., $f$ is the representation of $\varphi$ in $H$.

\paragraph{The mean map to probability distribution with respect to kernel} 
\begin{equation}\mu^{k(\cdot, \cdot)}(P_x) = E_{x\sim P_x} [k(x,\cdot)] = E_{x\sim P_x} [\phi(x)]_H \in RKHS
\end{equation} 
where "bra" $k(x,\cdot)$ is parameterized by $x$ and being integrated by $P_x$ as an 'average' function in RKHS.
\begin{itemize}
  \item $\langle \mu(P_x), f(\cdot)\rangle = E_{x\sim P_x}[f(x)]$
  \item if we know the "coordinate" of $\mu(P_x)$ and function $f(\cdot):\mathcal{X}\rightarrow \mathcal{R}$ in RKHS, then the expectation $E_{x\sim P_x}[f(x)]$ could be written as inner product in RKHS.
\end{itemize}

\section{MMD: Maximum Mean Discrepancy}
$MMD^{\mathcal{F}}(P_x, P_y) = \underset{f\in \mathcal{F}}{\sup} E_{P_x} [f(x)]- E_{P_y}[f(y)]$: to find a function $f$ that makes the difference of the mean of this function maximum.

If we constrain the Function space $F$ to be in the unit ball of a Hilbert Space, we do not need to superior operation anymore.

\begin{align}
  &MMD^{\mathcal{F}}(P_x, P_y) \\
  =& \underset{f \in \mathcal{F}, ||f||\le 1}{\sup} E_{P_x} [f(x)]- E_{P_y}[f(y)]\\
                              =&\underset{f \in \mathcal{F}, ||f||\le 1}{\sup} E_{P_x} [\langle w_f, \phi(x)\rangle]- E_{P_y}[\langle w_f, \phi(y)\rangle]\\
                              =&\underset{f \in \mathcal{F}, ||f||\le 1}{\sup} \langle w_f, E_{P_x} [\phi(x)]\rangle- \langle w_f, E_{P_y}[\phi(y)]\rangle]\\
                              =&\underset{f \in \mathcal{F}, ||f||\le 1}{\sup} \langle w_f, \mu^k(P_x)\rangle- \langle w_f, \mu^k(P_y)\rangle]\\
                              =&\underset{f \in \mathcal{F}, ||f||\le 1}{\sup} \langle w_f, \mu^k(P_x)-\mu^k(P_y)\rangle\\
\end{align}
since \begin{align}
 &|\langle w_f, \mu^k(P_x)-\mu^k(P_y)\rangle|^2 \\
&\le \langle w_f,w_f\rangle\langle \mu^k(P_x)-\mu^k(P_y), \mu^k(P_x)-\mu^k(P_y)\rangle\\
&\le \langle \mu^k(P_x)-\mu^k(P_y), \mu^k(P_x)-\mu^k(P_y)\rangle
\end{align} 
with equality at $\langle w_f,w_f\rangle\ = 1$

\begin{align} 
  &|MMD^{\mathcal{F}}(P_x, P_y)|^2 \\
  =&\underset{f \in \mathcal{F}, ||f||\le 1}{\sup} \langle w_f, \mu^k(P_x)-\mu^k(P_y)\rangle\\
  =&\langle \mu^k(P_x)-\mu^k(P_y), \mu^k(P_x)-\mu^k(P_y)\\
  =&||\mu^k(P_x)-\mu^k(P_y)||^2_H
\end{align}
\subsection{Moment matching property}
Let $\phi(x) = x$, then $\mathcal{X}$, as well as the RKHS be $R^d$, then $\mu^k(P_x)-\mu^k(P_y) = E_{P_x}x-E_{P_y}y$
Let $\phi(x) = (x, x^2)$, then 
$\sqrt{(E X - E Y)^2 + (E X^2 - E Y^2)^2}$ % https://stats.stackexchange.com/questions/276497/maximum-mean-discrepancy-distance-distribution

if $\mathcal{X} = R^d$ but $\mathcal{H}=R^p$, with $\phi(x) = Ax$, if $p<d$, then some distributions are not distingushable.

\subsection{Calculation of MMD2}
\paragraph{Method 1: unbiased}
\begin{align}
  &||\mu^k(P_x)-\mu^k(P_y)||^2_H \\
  =& \langle\mu^k(P_x)-\mu^k(P_y), \mu^k(P_x)-\mu^k(P_y)\rangle \\
  =& \langle\mu^k(P_x), \mu^k(P_x)\rangle+\langle \mu^k(P_y), \mu^k(P_y)\rangle + \\
  & \langle\mu^k(P_x), -\mu^k(P_y)\rangle +\langle -\mu^k(P_y), \mu^k(P_x)\rangle \\
  =&E_{P_x}E_{P_x}\langle k(x,x)\rangle +E_{P_y}E_{P_y}\langle k(y,y)\rangle \\
  &- E_{P_x}E_{P_y}\langle k(x,y)\rangle- E_{P_x}E_{P_y}\langle k(y,x)\rangle \\
  =&E_{P_x}E_{P_y}\langle k(x,x)\rangle +E_{P_x}E_{P_y}\langle k(y,y)\rangle \\
  & - E_{P_x}E_{P_y}\langle k(x,y)\rangle- E_{P_x}E_{P_y}\langle k(y,x)\rangle \\
  =&E_{P_x}E_{P_y} \left[\langle k(x,x)\rangle + \langle k(y,y)\rangle - \langle k(x,y)\rangle- \langle k(y,x)\rangle \right]
\end{align}

To estimate above, we draw samples from $P_xP_y$ assuming they are independent.
Draw $z_i = (x_i, y_i)$ and $z_j = (x_j,y_j)$, 
then the last equation could be estimated by 

\begin{align}
&\frac{1}{M^2}\sum_{i=1:M, j=1:M}\left[\langle k(x_i,x_j)\rangle + \langle k(y_i,y_j)\rangle - \langle k(x_i,y_j)\rangle- \langle k(y_i,x_j)\rangle \right]\\
  =&\frac{1}{M^2}\sum_{i\neq j}\left[\langle k(x_i,x_j)\rangle + \langle k(y_i,y_j)\rangle - \langle k(x_i,y_j)\rangle- \langle k(y_i,x_j)\rangle \right]\\ 
   &+\frac{1}{M^2}\sum_{i=j=1:M}\left[\langle k(x_i,x_i)\rangle + \langle k(y_i,y_i)\rangle - \langle k(x_i,y_i)\rangle- \langle k(y_i,x_i)\rangle \right]\\
  \approx &\frac{1}{M^2}\sum_{i\neq j}\left[\langle k(x_i,x_j)\rangle + \langle k(y_i,y_j)\rangle - \langle k(x_i,y_j)\rangle- \langle k(y_i,x_j)\rangle \right]
\end{align}
where the diagnal terms are ommited since there are only M number of them, while the other terms has a number of $M^2$
use this estimator when data come in pairs $z_i =(x_i, y_i)$ and you have to estimate a sample of 
$z_1, z_2, \ldots, z_M$



\paragraph{Kernel, Gram Matrix and the negative MMD2 problem due to unbiased estimator}
We use composite kernel as super-position of Gaussian Kernels:
$k(x, x') = \sum_{j=1}^K e^{-\alpha_j\|x - x'\|^2}$, which means for identical terms $k(x,x) = K$

Suppose we stack observations and divide the matrix into four partitions. then 

\begin{equation}\frac{1}{M^2}\sum_{i=j=1:M}\left[\langle k(x_i,x_i)\rangle + \langle k(y_i,y_i)\rangle - \langle k(x_i,y_i)\rangle- \langle k(y_i,x_i)\rangle \right]
\end{equation}
is the trace of 4 submatrices.
\begin{align}
&G(x_1,\dots, x_n)\\
=&\begin{vmatrix} 
  \langle x_1,x_1\rangle & \langle x_1,x_2\rangle &\dots & \langle x_1,x_n\rangle, &\langle x_1,y_1\rangle & \langle x_1,y_2\rangle &\dots & \langle x_1,y_n\rangle\\
  \langle x_2,x_1\rangle & \langle x_2,x_2\rangle &\dots & \langle x_2,x_n\rangle, &\langle x_2,y_1\rangle & \langle x_2,y_2\rangle &\dots & \langle x_2,y_n\rangle\\
  \vdots&\vdots&\ddots&\vdots &\vdots&\vdots&\ddots&\vdots\\
  \langle x_n,x_1\rangle & \langle x_n,x_2\rangle &\dots & \langle x_n,x_n\rangle &\langle x_n,y_1\rangle & \langle x_n,y_2\rangle &\dots & \langle x_n,y_n\rangle\\\
%%%%%
  \langle y_1,x_1\rangle & \langle y_1,x_2\rangle &\dots & \langle y_1,x_n\rangle &\langle y_1,y_1\rangle & \langle y_1,y_2\rangle &\dots & \langle y_1,y_n\rangle\\
  \langle y_2,x_1\rangle & \langle y_2,x_2\rangle &\dots & \langle y_2,x_n\rangle &\langle y_2,y_1\rangle & \langle y_2,y_2\rangle &\dots & \langle y_2,y_n\rangle\\
  \vdots&\vdots&\ddots&\vdots &\vdots&\vdots&\ddots&\vdots\\
  \langle y_n,x_1\rangle & \langle y_n,x_2\rangle &\dots & \langle y_n,x_n\rangle &\langle y_n,y_1\rangle & \langle y_n,y_2\rangle &\dots & \langle y_n,y_n\rangle
\end{vmatrix}
\end{align}
Note the absence of the cross terms  $- \langle k(x_i,y_i)\rangle- \langle k(y_i,x_i)$ from the off-diagnal submatrix's traces.
So 
\begin{align}
  &\hat{MMD2} = \frac{1}{M*(M-1)}sum(K_{xx})-trace(K_{xx})\\
   &+ sum(K_{yy}) - trace(K_{yy})- 2*sum(K_{x,y}) + 2*trace(K_{x,y})
\end{align}



\paragraph{Method 2: positive biased}
If we have two independent samples of $(x_1, x_2, \ldots, x_M)$ and $y_1, y_2, \ldots, y_M$ where we could compare any two items in the two samples (in Method 1 we also compute cross terms but we ommit the self cross)
.

Still we do not want the following superium operation:
\begin{align}
  MMD^{\mathcal{F}}[p,q] = \underset{f\in \mathcal{F}}{sup}E_{p_x} [f(x)] - E_{p_y}[f(y)]
\end{align}
\begin{align}
  \hat{MMD}^{\mathcal{F}}[p,q] = \underset{f\in \mathcal{F}}{sup} \frac{1}{m}[\sum_{i=1:M}f(x_i)] - \frac{1}{N}[\sum_{j=1:N}[f(y_j)]
\end{align}
Instead, first estimate $\mu^k(P_x)$ and $\mu^k(P_y)$

$\hat{\mu}^k(P_x) = \frac{1}{M}[\sum_{i=1:M}k(x_i, \cdot)]$ 

$\hat{\mu}^k(P_y) = \frac{1}{N}[\sum_{j=1:N}k(y_j, \cdot)]$ 

so
\begin{align}
  &\hat{MMD2}^{\mathcal{F}}[p,q] \\
  &=||\mu^k(P_x)-\mu^k(P_y)||^2_H \\
  &= \frac{1}{M^2}\sum_{i=1:M,j=1:M} k(x_i,x_j) +\frac{1}{N^2}\sum_{i=1:M,j=1:N} k(y_i,y_j) - \frac{2}{MN}\sum_{i=1:M, j=1:N}k(x_i,x_j)
\end{align}


==> cover_letter.tex <==
%\centering{
MLJ contribution information sheet%}
\begin{itemize}
\item What is the main claim of the paper? Why is this an important contribution to the machine learning literature?
["We are the first to have done X" is not an acceptable answer without stating the importance of X.]\\
\textbf{Answer}: \\
Domain-unsupervised domain generalization is essential since in many real world use cases it is difficult to assign distinct domain labels to different data sources assuming they have a equal domain distance. 
We proposed a novel domain generalization method based on hierarchical variational auto-encoding for domain-unsupervised generalization. Our method deals with hierarchical, sequential (near continuous) and overlapped domain shift which is less well studied in the domain generalization community compared to clearly separated domains. Our method shows favorable performance compared to state-of-the-art on both the clearly separated domains and the more complex domain settings.  \\

\item What is the evidence you provide to support your claim? Be precise.
["The evidence is provided by experiments and/or theoretical analysis" is not an acceptable answer without a summary of the main results and their implications.]\\
\textbf{Answer:}\\
On the domain generalization benchmark PACS, with an AlexNet architecture, our methods wins several state-of-the-art algorithms. On a real world medical image classification task as well as 3 synthetic domain generalization scenario with hierarchical, sequential (near continuous) and overlapped domain shift, our method also excels. \\
\item What papers by other authors make the most closely related contributions, and how is your paper related to them?
Have you published parts of your paper before, for instance in a conference? If so, give details of your previous paper(s) and a precise statement detailing how your paper provides a significant contribution beyond the previous paper(s). 
\\
\textbf{Answer}:\\
"DIVA:Domain Invariant Variational Autoencoders, Ilse, et.al." is another variational auto-encoding based domain generalization algorithm. However, their algorithm relies on explicit domain label assuming the domain distance between different data sources are equal which is not necessarily the case in real world scenarios. Our method is domain-unsupervised instead. Since our model is  hierarchical, the inference is more complicated. Our method mitigate several limitations of DIVA on hierarchical, sequential (near continuous), and overlapped domain shift scenarios. Our method has better disentanglement of variances on complex domain setting compared to DIVA. %Besides, we did ablation study on different latent variable $z_x$. \\
\\
This submitted paper is not yet published in any conferences nor journals. 
\end{itemize}

==> errata.tex <==
\section{Erratum on Mnist-Overlap}\label{sec:errta}
We correct a mistake occurring in Table \ref{tb:mnist-overlap} due to erroneously filling in the table with a value from another setting.
The correct result is in the new table in Table \ref{tb:mnist-overlap-erreta} where we do not find any statistical performance difference between the two algorithms under this overlapped rotated mnist scenario. It can be the case that the overlapped setting is challenging for both DIVA and HDIVA so it is difficult to show the advantages of HDIVA. However, we are able to show HDIVA outperforms DIVA in a more realistic domain overlapped experiment in section \ref{sec:cont_overlap}, so that our conclusion regarding the advantage of HDIVA under overlapping domain shift remains intact.
\begin{table}[h!]
	\centering
	\begin{tabular}{ |p{3cm}||p{2cm}|p{2cm}|}
		\hline
		Algorithm  & DIVA &  HDIVA  \\
		\hline
		Accuracy  & 0.821 $\pm$ 0.007    & 0.821 $\pm$ 0.007 \\
		\hline
	\end{tabular}\caption{The overlapped Rotated MNIST scenario where the first nominal domain contains rotations of 15, 30, 45 degrees and the second nominal domains contains rotation angles of 30, 45, 60, both algorithms train on two nominal domains and test on out of domain rotation angles at 0, 22, 75 respectively and we report the average accuracy with standard deviation by averaging results from 10 random seeds. The test set is taken from all 60k MNIST samples and rotate them by the angles respectively.}
	\label{tb:mnist-overlap-erreta}
\end{table}

==> eval.tex <==
\subsection{Evaluation Scheme}
\paragraph{Neural Style Transfer for Adversarial Learning}
%$Minkowski(X,Y) = (|x_i-y_i|^p)^{\frac{1}{p}}$
\paragraph{Evaluation scheme}
Current DG evaluation works on leave one out, which means training on all but one available domains and use the left out as test dataset. Rather than setting such a single point evaluation scenario to compare different algorithms, we propose to construct a sequence of distributions with increasing shift, and evaluate the area under curve.

==> iclr_malaria_detail.tex <==
\section{Further detail about experiment setting of the virtual malaria hospital}\label{sec:iclr_malaria_supp}
Virtual hospital C6 has 10 patients with 1061 infected cell images (in total 1748 images). Virtual hospital C8 has 10 patients with  957 infected cell images (in total 1638 images).  Virtual hospital C9 has 10 patients with 1284 infected cell images (in total 1964 images). Virtual hospital C1 has 90 patients with 8023 infected cell images (in total 14190 images). Each time, we combine the C6, C8, C9 virtual hospital domain as 3 training domains and sample 20 percent of the images for training. 20 random repetitions are done.  We report result on the test domain corresponding to virtual hospital C1.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> para_data_generation_process_factorization.tex <==
\paragraph{Data Generation Process}
\begin{align}
 &\prod_{l=1:L}\prod_{i=1:N^{(l)}}\prod_{j=1:M^{(l)}}p(x^{l,i,j},s^{l,i},z_x^{l,i,j},z_y^{l,i,j},z_d^{l,i,j},y^{l,i,j},\\
 \alpha^{l})
&=\prod_{l=1:L}\prod_{i=1:N^{(l)}}\prod_{j=1:M^{(l)}}\nonumber\\
&p(s^{(l,i)}|\alpha^{(l)})p(z^{(l,i,j)}_{d}|s^{(l,i)})p(x^{(l,i,j)}|z_x^{(l,i,j)},z_y^{(l,i,j)},z_d^{(l,i,j)})\\
&p_x(z_x^{l,i,j})p(z_y^{(l,i,j)}|y^{(l,i,j)})p_y(y^{(l,i,j)})
\end{align}
\paragraph{Marginal Distribution $p(x)$}
\begin{align}
&\prod_{l=1:L}\prod_{i=1:N^{(l)}}\prod_{j=1:M^{(l)}}p(x^{l,i,j})=E_{s,z_x,z_y,z_d}\\
&\left[\prod_{l=1:L}\prod_{i=1:N^{(l)}}\prod_{j=1:M^{(l)}}p(x^{l,i,j},s^{l,i},z_x^{l,i,j},z_y^{l,i,j},z_d^{l,i,j},y^{l,i,j},\alpha^{l})\right]
\end{align}
\paragraph{Factorization on variational posterior distribution}
\begin{align}
  &\prod_{l=1:L}\prod_{i=1:N^l} \prod_{j=1:M^l}q(z_d^{(l,i,j)}|\hat{\alpha}^{(l,i)}, s^{(l,i)}|x^{(l,i,j)}) \\
  &= \prod_{l=1:L}\prod_{i=1:N^l} q(s^{(i,l)}|z_d^{(i,l,j=1:M^l)})\prod_{j=1:M^l}q(z_d^{(i,l,j)}|x^{(i,l,j)}) \label{eq:varposdec}
\end{align}

==> para_dirichlet_merge_variable.tex <==
\paragraph{Properties of Dirichlet Distribution}
If $\theta=[X_1, X_2, \cdots, X_K]\sim Dir(\alpha_1,\alpha_2, \cdots, \alpha_K)$, then 
$\theta^{'}=[X_1, X_2, \cdots, X_{K-1}+ X_K]\sim Dir(\alpha_1 , \alpha_2, \cdots, \alpha_{K-1}+\alpha_K)$
note that
\begin{align}
&p(\theta^{'})\\
&=\sum_{X_{K-1}+X_K=X^{'}_{K-1}}Dir(X_1,X_2, \cdots, X_{K-1},X_{K}|\\
&\alpha_1, \alpha_2, \cdots, \alpha_{K-1}, \alpha_{K})
\end{align}
 

==> para_kl_divergence_hierarchy.tex <==
\paragraph{KL divergence}
For each domain $l$, batch $i$, we could compute the KL divergence of the `topic' $s^{(l,i)}$:
\begin{align}
&D_{kl}^{(k)}(q(s^{(l,i)}|z^{(l,i)}_{d_{1:M}})||p(s^{(l,i)}|\alpha))\\
&D_{kl}^{(k)}(q(z_d^{(l,i)}|x^{(l,i)})||p(z_d^{(l,i)}|s^{(l,i)}))
\end{align}

\paragraph{KL divergence on hierarchical DAG}
Consider an arbitrary chain with two levels, $z_2 -> z_1 -> x$, we have
\begin{align}&KL(q(z_1,z_2|x)|p(z_1,z_2))\\ 
&= E_{q(z_1,z_2|x)}\log\frac{q(z_1,z_2|x)}{p(z_1,z_2)}\\
&=E_{q_1(z_1|x)q_2(z_2|z_1,x)}\log\frac{q_1(z_1|x)q_2(z_2|z_1,x)}{p_1(z_1|z_2)p_2(z_2)}\\
&=E_{q_1(z_1|x)}E_{q_2(z_2|x,z_1)}\left[\log\frac{q_1(z_1|x)}{p_1(z_1|z_2)}+ \log\frac{q_2(z_2|z_1,x)}{p_2(z_2)}\right]\\
&=E_{q_1(z_1|x)}\left[ E_{q_2(z_2|x,z_1)}\log\frac{q_1(z_1|x)}{p_1(z_1|z_2)}+ E_{q_2(z_2|x,z_1)}\log\frac{q_2(z_2|z_1,x)}{p_2(z_2)}\right]\\
&= E_{q_1(z_1|x)}\left[ E_{q_2(z_2|x,z_1)}\log\frac{q_1(z_1|x)}{p_1(z_1|z_2)}\right] +  E_{q_1(z_1|x)}KL(q_2(z_2|z_1,x)||p_2(z_2))
%&=E_{q_2(z_2|x,z_1)}KL(q_1(z_1|x)||p_1(z_1|z_2)) + E_{q_1(z_1|x)}KL(q_2(z_2|z_1,x)||p_2(z_2))
\end{align}
Substitute $z_1=z_d$ and $z_2=s$ in our model, and  assume \begin{equation}
q(z_d,s|x) = q_1(z_d|x)q_2(s|z_d,x)=q_1(z_d|x)q_2(s|z_d)
\end{equation}, we have $p(z_d, s|\alpha)=p(z_d|s)p(s|\alpha)$
\begin{align}
&KL(q(z_d,s|x)|p(z_d,s|\alpha))\\
%&=E_{q_{\phi_s}(s|x,z_d)}KL(q_1(z_d|x)||p_1(z_d|s)) + E_{q_{\phi_d}(z_d|x)}KL(q_{\phi_s}(s|z_d,x)||p_2(s|\alpha))\\
 &=E_{q_{\phi_s}(s|x,z_d), q_{\phi_d}(z_d|x)}\frac{q_{\phi_d}(z_d|x)}{p_{\theta_d}(z_d|s)} + E_{q_{\phi_d}(z_d|x)}KL(q_{\phi_s}(s|z_d)||p_{\theta_s}(s|\alpha)) \label{eq:hkl}
\end{align}
\textbf{The first part of Equation \ref{eq:hkl} is a R.V. conditioned on $s$ at the particular batch and sampled topic, the second part is a double integration with both $z_d$ and $s$ and does not depend on particular value of $z_d$ or $s$. }


==> para_nll.tex <==
\subsubsection{Different $E_{q(z)}\log p(x|z)$ reconstruction loss}
\begin{itemize}
\item Gaussian: $E_{q(z)}\log p(x|z) = E_{q(z)} [\sum_{i,j}-0.5 \frac{(x_{i,j}-\mu_{i,j}(z))^2}{\sigma_{ij}^2(z)}-0.5\log\sigma^2]$
\item Logistic256: $E_{q(z)}\log p(x|z) =-\log [\sigma\left( \frac{[x_{ij}*256]/256 - \mu_{i,j}(z)}{\sigma_{ij}^2(z)} + \frac{1}{256 \sigma_{ij}^2(z)}\right) -\sigma\left( \frac{[x_{ij}*256]/256 - \mu_{i,j}(z)}{\sigma^2_{ij}(z)} \right) + \epsilon]$
\end{itemize}

==> poster_conc.tex <==
\begin{itemize}
\item Our approach does not require observed domain labels during training, facilitating domain generalization for a much wider range of applications. Additionally, our approach does not need validation set for model selection but only use extended ELBO for model selection.
\item In the presence of domain-substructure, our algorithm is able to robustly disentangle domain-specific variation from class-label specific variation. 
\item Our algorithm is able to model domain overlap via interpretable topics and generalize to settings with continuous domain shift. 
\item Our algorithm has a competitive performance even in standard domain generalization tasks, where observed domain information is available on clearly separated domains. 
\item We proposed evaluation dataset for benchmarking hierarchical and sequential domain shift.
\end{itemize}

==> poster_fig_diverge_seq_overlap_mnist_color.tex <==
\begin{figure}[H]
	\centering
		\subfloat[]{\includegraphics[width=0.15\textwidth]
			{../figures/mnist_color_cont_combo_domain_ind0.png}\label{fig:seq_overlap_combo0}}
		%\hfil
		\subfloat[]{\includegraphics[width=0.15\textwidth]{../figures/mnist_color_cont_combo_domain_ind1.png}\label{fig:seq_overlap_combo1}}
		\subfloat[]{\includegraphics[width=0.15\textwidth]{../figures/mnist_color_cont_combo_domain_ind2.png}\label{fig:seq_overlap_combo2}}
	%\includegraphics[width=0.4\textwidth]{temp4img/color_cont_diverge_back_diverge_hue_0_350_fore_hls.png}
	%\caption{\textbf{Sequential Color-Mnist (Red Diverging Palette)}.
	%Background color taking 7 hue values spanning in the area between 0 and 350 hue degrees (red spectrum) sequentially, with fixed saturation and lightning, foreground color takes equally spaced hue value in the complete hue circle with fixed saturation and lightning. Background and foreground colors are zipped. The first 3 color schemes representing 3 sub-domains compose the first nominal domain in Fig. \ref{fig:seq_overlap_combo0}, the 2nd nominal domain take the middle 3 color schemes with one color scheme overlap with the 1st and another color scheme overlap with the 3rd nominal domain in Fig. \ref{fig:seq_overlap_combo1}. The 2nd nominal domain serves as a bridge between the other two nominal domains. Out of domain test accuracy is reported in Table \ref{tb:red-diverging-seq_color_overlap}.}
	\label{fig:red-diverging-color-mnist-seq-overlap}
\end{figure}

==> poster_fig_double_color_mnist.tex <==
\begin{tikzfigure}[Color combination of as Hierarchical Domains]
\centering
\begin{minipage}{0.2\textwidth}
\includegraphics[]
{../figures/mnist_color_combo_domain_ind0.png}\label{fig:combo0}
\end{minipage}
%\hfil
\begin{minipage}{0.2\textwidth}
	\includegraphics[]{../figures/mnist_color_combo_domain_ind1.png}\label{fig:combo1}
\end{minipage}
\begin{minipage}{0.2\textwidth}
\includegraphics[]{../figures/mnist_color_combo_domain_ind2.png}\label{fig:combo2}
\end{minipage}
%\captionof{figure}{\textbf{Random combination of Color-Mnist as Hierarchical Domains}. Mnist has both its foreground and background colored, each color combination represent one sub-domain. Each nominal domains include 2 sub-domains.}
\label{fig:color_mnist_both_combo}
\end{tikzfigure}


==> poster_seq_color_overlap_vlag.tex <==
\begin{table}[H]
	\centering
	%\caption{ \textbf{Out of Domain Accuracy for Color-Mnist (VLAG Palette) in Figure \ref{fig:vlag-color-mnist-cont-overlap}}. Each sub-domain in Figure \ref{fig:vlag-color-mnist-cont-overlap} contains a random sample of 1000 mnist images. Random seed is shared for the different sub-domains of a nominal domain but different across nominal domains. Each repetition is with different starting random seed, 10 repetitions are done. The sub-domains are combined to form one nominal domain and 50 percent is used for training, the rest for validation. Comparison algorithms are DIVA \mcitep{ilse2019diva} and Match-DG \mcitep{mahajan2020domain}, while Deep-All is used as baseline by pooling all training domain s together. The 2nd domain is a bridge domain that connect the 1st and 3rd domain, so it is not used as test domain at all.  }
	%\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|  }
	\begin{tabular}{ p{5cm}cc }
		\toprule
		%\multicolumn{4}{|c|}{Style Digit} \\
		%\hline
		 \bfseries Color-Mnist (VLAG) & \bfseries Test Domain 1& \bfseries Test Domain 3 \\
		%\hline
		\midrule
		%DIVA(Elbo)
		%& 0.66 $\pm$ 0.06 & 0.67 $\pm$ 0.03 \\
		DIVA &0.63 $\pm$ 0.05 &0.68 $\pm$ 0.03 \\
		
		HDUVA & \textbf{0.69} $\pm$ 0.05 & \textbf{0.71} $\pm$ 0.03 \\
		
		Deep-All & 0.60 $\pm$ 0.05 & 0.68 $\pm$ 0.04 \\
		
		%CVAE & 0.69 0.03 & 0.70 0.04\\
		Match-DG  & 0.67 $\pm$ 0.06 &  0.70 $\pm$ 0.03\\
		\bottomrule
	\end{tabular}
	
	\label{tb:vlag-seq_color_overlap}
\end{table}

==> poster_tb_diverge_seq_overlap.tex <==
%\begin{table*}[!t]
\begin{table}[H]
	\centering
	%\caption{ \textbf{Out of Domain Test Accuracy for Sequential Color-Mnist (Red Diverging Palette) from Figure \ref{fig:red-diverging-color-mnist-seq-overlap}}. Each sub-domain in Figure \ref{fig:red-diverging-color-mnist-seq-overlap} contains a random sample of 1000 mnist images. Random seed is shared for the different sub-domains of a nominal domain but different across nominal domains. Each repetition is with different starting random seed, 10 repetitions are done.  The sub-domains are combined to form one nominal domain and 50 percent is used for training, the rest for validation. Comparison algorithms are DIVA \mcitep{ilse2019diva} and Match-DG \mcitep{mahajan2020domain}, while Deep-All by pooling all training domains together is used as baseline. The 2nd domain is a bridge domain that connect the 1st and 3rd domain, so it is not used as test domain at all.}
	%\begin{tabular}{ p{2cm}p{2cm}p{2cm}  }
	\begin{tabular}{ p{6cm}cc }
		\toprule
		%\multicolumn{4}{|c|}{Style Digit} \\
		%\hline
		\bfseries Color-Mnist (Red Diverge %#\quad\quad\quad\quad(red background
)  & \bfseries Test Domain 1 &  \bfseries Test Domain 3 \\
	    \midrule
		%DIVA         &  0.603 $\pm$ 0.04   & \textbf{0.464 $\pm$ 0.02}
		 %&  0.959 $\pm$ 0.002\\
		%HDIVA   & \textbf{0.653 $\pm$ 0.04}   &0.453 $\pm$ 0.03  &  \textbf{0.975 $\pm$ 0.008}   \\
		%DIVA(elb) &0.51 $\pm$ 0.04 & 0.65 $\pm$ 0.06 \\
		DIVA &0.53 $\pm$ 0.05 & 0.63 $\pm$ 0.05 \\
		\mname{} & \textbf{0.56} $\pm$ 0.05 & \textbf{0.68} $\pm$ 0.05 \\
		
		Deep-All &0.53 $\pm$ 0.06 &0.61 $\pm$ 0.06 \\
		
		%LHDIVA  & 0.52 0.04 & 0.67 0.02\\
		%\hline
		Match-DG  & 0.44 $\pm$ 0.04 &  0.67 $\pm$ 0.10\\
		\bottomrule

	\end{tabular}
	\label{tb:red-diverging-seq_color_overlap}
\end{table}
%\vspace*{\fill}

==> poster_tb_pacs.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\usepackage{geometry}
%\usepackage{array}

%\usepackage{multirow}
%\usepackage{booktabs}
%\usepackage{threeparttablex}
%\usepackage[table]{xcolor}



%\begin{document}

\begin{table}[H]
	\centering
	\small
	%\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}
		\caption[Domain Generalization in PACS Dataset with AlexNet]{\textbf{Domain Generalization in PACS Dataset with AlexNet Classifier}}
		\begin{tabular}{llllll}
			\toprule
			\bfseries Methods 	      & \bfseries Art Painting &  \bfseries Cartoon & \bfseries	Photo & \bfseries Sketch & \bfseries  Ave.   \\
			\midrule
                  Jigsaw    &   \underline{46.90} $\pm$ 1.23            &  51.85 $\pm$ 2.08     &  66.96 $\pm$ 1.19               &  \textbf{65.28 $\pm$ 3.72}   &  57.75   \\
                  Jigsaw(Caffe)    &  64.20 $\pm$ 1.34            &  66.08 $\pm$ 0.39     &  89.51 $\pm$ 0.51               &  62.32 $\pm$ 0.85   &  70.53   \\
                  %MatchDG(reported)     &0.67 $\pm$0.01 & 0.69 $\pm$ 0.01 &0.89 $\pm$ 0.01 &0.63 $\pm$ 0.02 & 0.72\\
                  MatchDG     &0.67 $\pm$0.01 & 66.64 $\pm$ 0.98 &0.89 $\pm$ 0.01 &0.63 $\pm$ 0.02 & 0.72\\
                  %DIVA \cite{ilse2019diva} &  47  & 58    &68    &56 &57.25\\ 
                  %DIVA-AUG      &  50  & 68    & 73   & 43 &58.5 \\
                  %DIVA(elbo)    & 0.66 $\pm$ 0.01   & 0.68 $\pm$ 0.03 &  0.88  & 0.61 0.02 \\
                   DIVA    & 0.64 $\pm$ 0.02    & 0.66 $\pm$ 0.003 &  0.87 $\pm$ 0.01 & 0.58 $\pm$ 0.03 & 0.69 \\
                    Deep-All & 0.64 $\pm$ 0.01 &  0.67 $\pm$ 0.02 &  0.85 $\pm$ 0.02  &  0.56 $\pm$ 0.02 & 0.68 \\
                  \mname{}  & 0.65 $\pm$ 0.01  & 0.66 $\pm$ 0.01 &  0.87 $\pm$ 0.01  & 0.58 $\pm$ 0.01 & 0.69 \\
                  W\mname{}$^{\ast}$ &  0.64 $\pm$ 0.01  & 0.67 $\pm$ 0.02 & 0.88 $\pm$ 0.01 & 0.60 $\pm$ 0.02 & 0.70\\
                 \mname-no-zx$^{\ast\ast\ast\ast}$ &0.65$\pm$ 0.01 & 0.67$\pm$0.02 & 0.87 $\pm$ 0.01 & 0.61 $\pm$ 0.03 &0.70\\
                 % Sketch(8, 0.6076602, 0.02745811), photo(7, 0.8724675, 0.01425576), cartoon(8, 0.6663462, 0.01720015), art-painting(7, 0.6514706, 0.009921686)
                  L\mname$^{\ast\ast}$ & 0.65 $\pm$ 0.003  & 0.69 $\pm$ 0.02   & 0.87 $\pm$ 0.004 & \underline{0.55 $\pm$ 0.002} & 0.69 \\
                  \mname-CTR$^{\ast\ast\ast}$ & 0.65 $\pm$ 0.01  & 0.66 $\pm$ 0.02   & 0.88 $\pm$ 0.01 &  0.63 $\pm$ 0.003 & 0.71 \\
                  %HDIVA     &  56  & 62    &75   & 56 &62.25 \\
                  %HDIVA-AUG  &54  & 64  &82   & 60 & 65 \\
			\bottomrule
		\end{tabular}
		
		\begin{tablenotes}
			\item  %Variants of our algorithm in the table:\\
			$^{\ast}$ W\mname: weak domain-supervision added to \mname{} as explained  in Appendix \ref{sec:weak}.\,\,\\ $^{\ast\ast}$L\mname: Ladder \fullalgoname explained in Appendix \ref{sec:lhdiva}.\\
			$^{\ast\ast\ast}$\mname-CTR: Use the contrastive learning phase (pretrain phase) of \mcitet{mahajan2020domain} as initialization for AlexNet of \mname.\\
			$^{\ast\ast\ast\ast}$\mname-no-zx: \mname{} without $z_x$ variable, see Figure~\ref{fig:hduva_no_zx}.%\\
			%Part of the table is adapted from \url{https://domaingeneralization.github.io/}.
		\end{tablenotes}
		\label{tb:pacs}
	\end{threeparttable}
\end{table}

%\end{document}


==> poster_vlag_overlap.tex <==
 \begin{tikzfigure}[Color combination of as Hierarchical Domains]
 \begin{minipage}{0.2\linewidth}
\includegraphics[]
			{../figures/mnist_color_seq_combo_overlap_domain_vlag_ind0.png}%\label{fig:vlag-combo0}
		%\hfil
	\end{minipage}
\begin{minipage}{0.2\linewidth}
\includegraphics[]{../figures/mnist_color_seq_combo_overlap_domain_vlag_ind1.png}%\label{fig:vlag-combo1}
\end{minipage}
\begin{minipage}{0.2\linewidth}
\includegraphics[]{../figures/mnist_color_seq_combo_overlap_domain_vlag_ind2.png}%\label{fig:vlag-combo2}
\end{minipage}
\end{tikzfigure}

==> sec_ablate.tex <==
\section{Ablation study}
We proposed two techniques for weak domain supervision, and investigate in this section the role each weak domain supervision technique plays. We repeated experiment \ref{sec:color-combo} on HDIVA with the only amendment that we choose four settings: Weak domain supervision with both MMD \ref{sec:mmd} and Topic distribution aggregation \ref{sec:agg_alpha} which we name \textbf{Agg-MMD}. Similarly, we have \textbf{no-Agg-MMD}, \textbf{Agg-no-MMD} and \textbf{no-Agg-no-MMD}. The last case, \textbf{no-MMD-no-Agg}, is a completely domain unsupervised setting.



\begin{table}[h!]
	\centering
	\begin{tabular}{ |p{3cm}||p{2cm}|p{2cm}|}
		\hline
		Weak Domain Supervision  & Flat-Prior &  Edge-Prior  \\
		\hline
		Agg-MMD  & 0.9217 $\pm$ 0.025    & 0.9114 $\pm$ 0.036 \\
		\hline
		no-Agg-MMD  & 0.9140 $\pm$ 0.031    & 0.9227 $\pm$ 0.034 \\
		\hline
		Agg-no-MMD  & 0.9236 $\pm$ 0.025    & 0.9041 $\pm$ 0.033 \\
		\hline
		no-Agg-no-MMD  & 0.9221 $\pm$ 0.026    & \textbf{0.9259} $\pm$ 0.025   \\
		\hline
	\end{tabular}\caption{}
	\label{tb:ablate}
\end{table}

==> sec_domain_semisup.tex <==
\section{Domain-Label semi-supervised Learning}\label{sec:semi_sup}
\input{tb_semi}
\input{tb_mnist_r}
\input{tb_semi_pacs}
If we get access to data from an unknown domain, which might consist of a mixture of existing domains, %\cite{matsuura2020domain}. 
it is favorable to utilize  these data in a domain-label-unsupervised manner. This is different from the existing class-label-semi-supervised learning where there is both instances with class labels and without class labels. We leave the combination of class-label and domain-label semi-supervised learning as future work. In this work, to show HDIVA can deal with domain-label-semi-supervised learning, based on Experiment \ref{sec:color-combo}, we added additional 1000 random MNIST instances (see section \ref{supsec:hyper_exp_set} for sources of these random samples) with equal class distribution and colored them according to the first row of Figure \ref{fig:color_mnist_both_combo}. For these 1000 instances, we do not do weak supervision (described in section \ref{sec:weak}), but instead feed them into the variational inference process only with their class label.  The results are shown in Table \ref{tb:semi}. 


==> sec_ehdiva.tex <==
direct inference
how to concatenate $z_2, z_1$ map to x
x->z2
x->z1hx, z2-z1hz2,  (z1hx,z1hz2)->z2
      2)   recon
	      -  prior decomposition    p(z1,z2) = p(z1|z2)p(z2)
                  -  posterior decomposition  q(z1,z2) = q(z1|z2,x)q(z2|x)
                  -  KL(q(z1,z2)|p(z1,z2)) = 
E_{q(z1|z2,x)q(z2|x)} log[ q(z1|z2,x)q(z2|x)/p(z1|z2)p(z2)]
the easiest way to implement this KL divergence is to use
KL = -(log_p_z1 + log_p_z2 - log_q_z1 - log_q_z2) directly, instead of further mathematical derivation.

do we want to have complete recon with topic, domain to x or only from zd to x?


==> sec_exp_domain_embed.tex <==
\subsection{Domain Embedding}\label{sec:overlap}
Here, we investigate the ability of our approach to generate meaningful domain embeddings. To this end, we adapt the standard rotated MNIST benchmark \mcitep{ilse2019diva} by introducing an overlap between three nominal domains: for the first nominal domain, we use 1000 samples of MNIST and rotate them by 15, 30 and 45 degrees respectively. Thus, the first domain contains 3000 instances and each rotation angle constitutes one sub-domain. For the second domain nominal domain, we rotate the same subset of MNIST, by 30, 45 and 60 degrees respectively. In this way, each nominal domains has two rotation degrees of overlap corresponding to 2000 instances that have the same rotation. We use these 2 nominal domains for training, and simulate a sequential domain shift for testing with rotation angles of 0, 22 and 75 degrees. We sampled images from both nominal training domains as well the continuously shifted test domain and plot their topic distributions in Figure \ref{fig:overlap_topic}. We expect the topics of the training domains to overlap substantially, due to the shared rotation angles. We further expect for the topics of the test domain to span the entire range of topics from both training domains. Figure \ref{fig:overlap_topic}~illustrates that \mname{} indeed assigns similar domain topics to many instances from both training domains, while samples from the test domain span the entire range of topics. %\ref{fig:diva-pgm}.
\begin{figure}[h]
	\center\includegraphics[width=0.25\textwidth]{img_topics.pdf}
	\caption{Topic plot of  overlapped domains}\label{fig:overlap_topic}
\end{figure}

==> sec_exp_iclr.tex <==
\section{Empirical Evaluation}\label{sec:exp}
We conduct experiments, trying to answer the following questions:
\begin{itemize}
	\item 
Could \mname{} mitigate the limitations of standard supervised approaches for domain generalization in terms of domain-substructure or incomplete domain information? We conduct experiments based on a real-world dataset for the classification of Malaria patients. \\%We conduct experiments in Section~\ref{sec:color-combo}, Section~\ref{sec:cont_overlap} and Section~\ref{sec:overlap} to address these issues.\\
%\item 
%In complex scenarios with domain substructure, can \mname{} still robustly disentangle domain-specific variation from class-label specific variation? See details in Section~\ref{sec:color-combo}.\\
%	\item  
%We visualize topics from overlapping nominal domains to illustrate why \mname{} improves upon supervised approaches in Section~\ref{sec:overlap}.\\
	\item 
How does \mname{} perform under standard domain generalization benchmarks where information on clearly separated domain is available, compared with other state-of-the-art algorithms? See Section~\ref{sec:pacs}.
\end{itemize}
In addition we provide results from additional experiments in the supplement, where we use simulated data to further illustrate that our algorithm outperforms standard domain generalization approaches in case of incomplete domain information. In the supplement we also visualize topics from overlapping nominal domains to illustrate why \mname{} improves upon supervised approaches. %Additionally, our algorithm only use ELBO as model selection criteria, without using the validation set. 
\input{source/sec_exp_malaria}
\input{source/sec_exp_pacs}

==> sec_future.tex <==
\section{Future work}
\paragraph{Try out other data types with HDIVA} Like Neural Machine Translation, Graph data, Time Series, Gene Data, etc

\paragraph{Class Label Semisupervised Learning} We add extra data points to the training, with domain label, but without class label.  

\paragraph{Investigate the sub-optimal performance reason for domain Label Semisupervised Learning} 
\begin{itemize}
\item Use Tensorboard to generate individual loss term plots.
\item Investigate in depth othere domain-unsupervised methods like the AAAI 2020 Paper in order to find out what is the key factor of enabling domain-unsupervised learning.
\item Investigate in depth VAE based deep clustering methods in order to find out key factors of enabling domain-unsupervised learning.
\end{itemize}
\paragraph{Domain-Class-Label semisupervised learning} feed data x without domain and class label

\paragraph{Life long learning} 
\begin{itemize}
  \item Investigate standard lifelong learning benchmark and design appropriate evaluation process to investigate if HDIVA works in a life long setting. 
  \item Implement stick-breaking vae which seems to be an early work of lifelong learning but not really evaluated.
\end{itemize}

\paragraph{Causality based domain generalization} Investigate recent papers in depth and try to implement their algorithms and extend HDIVA with causality interpretation and/or potential breaking point to improve the performance of HDIVA.

\paragraph{HDIVA improvement}
\begin{itemize}
  \item Code optimization
  \item Make Pixel CNN work
  \item Try if the DRAW model works together with HDIVA.
\end{itemize}

\paragraph{Domain Generalization Library} Implement more algorithms, with documentation

\paragraph{Trustworthy Certificate} Develop different self-data-augmenting routines to evaluate an algorithm robustness against distribution shift. Design evaluation metrics for assessing the performance.
\begin{itemize}
\item Adversarial data augmentation with wasserstein distance constraint
\item Adversarial trained noise generator to synthetize shifted image
\end{itemize}


==> sec_methods_iclr.tex <==
\section{Methods and Technical Solution}\label{sec:method}
%We build on previous work using autoencoder-based models for for domain generalization \cite{kingma2013auto,ilse2019diva} and propose a Hierarchical Domain-Invariant Variational Autoencoder that we refer to as HDIVA. %We follow \cite{ilse2019diva} and use three independent latent representations to disentangle variability in inputs $X$ related to domain-specific sources, label-specific sources and residual variation. 
\input{source/sec_methods_problem_state}
\input{source/sec_methods_hdiva_overview}

%\input{source/sec_methods_prior}
%\input{source/subsec_ehdiva_inference}
%\input{source/subsec_ehdiva_elbo}
%\input{source/subsec_ehdiva_algo}


==> sec_prior_work_cluster.tex <==
\section{Previous work on clustering model}
\subsection{GMVAE}
In Figure \ref{fig:gmvae}, the $s$ is the cluster assignment variable.

In the generation pass, $s$ is sampled, and $s$ select from $K$ Gaussian mean and variances of $z_1$ generated by $z_2$. There is no need for $K$ passes.

In the inference pass, $s$ is not inferred explicitly, 
 

The "reconstruction" part loss.
\begin{align}
&E_{q(z_2|x)q(z_1|x)q(s|z_1,z_2)}\log p(x|z_1, z_2, s)\\
=&E_{q(z_2|x)q(z_1|x)q(s|z_1,z_2)}\log \frac{p(s)p(z_2)p(z_1|s,z_2)p(x|z_1)}{p(z_1,z_2,s)}\\
=&E_{q(z_2|x)q(z_1|x)q(s|z_1,z_2)}\log p(x|z_1)
\end{align}
The KL divergence
\begin{align}
&KL\left(q(z_1,z_2,s|x)||p(z_1,z_2,s)\right)\\
=&KL\left(q(z_2|x)q(z_1|x)q(s|z_1,z_2)||p(s)p(z_2)p(z_1|s,z_2)\right)\\
=&E_{q(z_2|x)q(z_1|x)q(s|z_1,z_2)}\log \left(q(z_2|x)q(z_1|x)q(s|z_1,z_2)\right) -\log\left(p(s)p(z_2)p(z_1|s,z_2)\right)\\
=&E_{q(z_2|x)q(z_1|x)q(s|z_1,z_2)} \log \frac{q(z_1|x)}{p(z_1|s,z_2)}+\log \frac{q(z_2|x)}{p(z_2)} + \log \frac{q(s|z_1, z_2)}{p(s)}\\
=&E_{q(z_2|x)q(s|z_1,z_2)}KL(q(z_1|x)||p(z_1|s,z_2)) + KL(q(z_2|x)||p(z_2))+\\
&E_{q(z_2|x)q(z_1|x)} KL(q(s|z_1,z_2)|p(s))  
\end{align}

\begin{figure}[h!]
	\center\includegraphics[width=0.4\textwidth]{tikz_gmvae_mix.pdf}
	\caption{GMVAE}
	\label{fig:gmvae}
\end{figure}



The problem of their method is $E_{q(z_2|x)q(z_1|x)} KL(q(s|z_1,z_2)|p(s))$, where $p(s)$ can not be an informative prior, therefore, the KL divergence term will tend to merge clusters so that $q(s|z_1,z_2)$ will be concentrated.


\subsection{Semi-supervised M2}

\begin{align}
p(x, y, z) &= p(y)p(z) p(x \mid y, z)\\
y &\sim \text{Cat}(1/K) \\
z &\sim \mathcal{N}(0, I) \\
x &\sim \mathcal{B}(\mu_x(y, z))\\
q_{\phi}(z|y,x) &= \mathcal{N}(z|\mu_{\phi}(y,x), diag(\sigma^2_{\phi}(x)))\\
q_{\phi}(y|x)&=Cat(y|\pi_{\phi}(x))
\end{align} 
The marginal posterior of $z$ can be written as 
\begin{align}
q(z \mid x) &= \sum_i q(z, y \mid x) \\
&= \sum_i q(y \mid x) q(z \mid x, y).\label{eq:m2-mixture}
\end{align}
Under unsupervised condition, if $H(y|x)=-\sum_x\sum_y q(y|x)\log q(y|x)$  is minimized, which means $y$ could encode information about $x$(i.e. the softmax vector of $q(y|x)$ is mostly concentrated in one bit), then equation \ref{eq:m2-mixture} is degrading to a single Gaussian, instead of a mixture of Gaussian with mixture coefficient $p(y|x)$.

\begin{figure}[h!]
	\center\includegraphics[width=0.4\textwidth]{tikz_m2.pdf}
	\caption{M2 NIPS 2015}
	\label{fig:gmvae}
\end{figure}


\subsection{VFAE ICLR 2016}
\begin{figure}[h!]
	\center\includegraphics[width=0.4\textwidth]{tikz_vfae.pdf}
	\caption{VFAE}
	\label{fig:gmvae}
\end{figure}

\subsection{DLGMM (NIPS2016 Workshop)}
Generation phase: (avoid sample cluster assignment variable) 
\begin{align}
\pi &\sim \text{DirichtletProcess}(\alpha_0) \text{ linear time stick breaking} \\
z   &\sim \sum_{1}^{K} \pi_k \mathcal{N}(\mu_k, \sigma_k) \text{ sample intractable}\\
x   &\sim  p_{\theta}(x|z) = \sum_{1}^{K} \pi_k p\left({x_k | z(\mu_k, \sigma_k)}\right) \text{ sample z for K times} 
\end{align}
"reconstruction" happens at each $x_k$.

Inference phase: 
assume component wise decomposition of GEM variable
\begin{align}
\hat{\pi_k} &\sim  Kumar_{\phi}\left(\hat{\pi_k} | a_k(x), b_k(x))\right)\\
\hat{z}   &\sim \sum_{1}^{K} \hat{\pi}_k \mathcal{N}_{\phi}(\hat{z_k}| \mu_k(x), \sigma_k(x))
\end{align} 

\begin{figure}[h!]
	\center\includegraphics[width=0.4\textwidth]{tikz_dlgmm.pdf}
	\caption{DLGMM NIPS 2016}
	\label{fig:gmvae}
\end{figure}


"Reconstruction" loss of ELBO:
\begin{align}
E_{\hat{\pi}_k, \hat{z_k}} \sum_{k=1}^{K}\hat{\pi_k}p(x_k=x|\hat{z_k}(x))
\end{align}

KL divergence part of ELBO: since there is no hierarchy structure, the KL divergence part is also simple

$KL(q(\pi)||p(\pi_1, \cdots, \pi_K))) = -\sum_{k=1}^{K} KL\left(\text{Kumar}_{\phi}\left(\hat{\pi_k} | a_k(x), b_k(x)\right) || p(\pi_k)\right)$ 

and 

\begin{align}
&-KL\left(q(z_1, \cdots, z_K, \pi_1, \cdots, \pi_K|| p(z_1, \cdots, z_K)\right) \\
=&\sum_{k=1}^{K}E_{z_1, \cdots, z_K, \pi_1, \cdots, \pi_K}p(z_k | \bar{\mu}_k, \bar{\sigma}_k) - \log \sum_{k=1}^{K}\pi_k q(z_k| \hat{\mu}_k(x), \hat{\sigma}_k(x))
\end{align}

\subsection{SB-VAE ICLR 2017}
Figure \ref{fig:sb-vae}
\begin{figure}[h!]
	\center\includegraphics[width=0.4\textwidth]{tikz_sb_vae.pdf}
	\caption{SB-VAE ICLR 2017}
	\label{fig:sb-vae}
\end{figure}




\begin{table*}[t]
	\centering
	\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}||p{2cm}| p{2cm} | }
	\hline
	\multirow{1}{*}{}
	&\multicolumn{2}{c}{Advantages} & \multicolumn{2}{c}{Disadvantage}  \\ 
    \hline
	Model v.s. Property  & Continuous Domain Shift & Large number of domains &  Multiple Pass &  Explicit Cluster Assignment\\
	\hline
	DSVAE(our's)   & Yes  & Yes  &  No  & No  \\ \hline
	DIVA   (ICLR 2019) & No  & No  &  No  & Yes  \\ \hline \hline
	SB-VAE (ICLR 2017)  & Yes  & Yes  &  No  & No  \\ \hline
	DLGMM (NIPS 2016)   & No  & No  &  Yes  & No  \\ \hline
	GMVAE (ICLR 2017)   & No  & No  &  Yes  & No  \\ \hline 
	M2 (NIPS 2014)      & No  & No  &  Yes  & No  \\ \hline
	VFAE (NIPS 2018)    & No  & No  &  Yes  & No  \\ 
    \hline
\end{tabular}
\caption{Comparison of Deep Clustering Method}
\label{tb:model_comparison}		
\end{table*}
%\lipsum[1-20]

==> sec_unsup.tex <==
\paragraph{Direct derivation}
\begin{align}
  q(z_y, y|x) = q(z_y|x) q(y|z_y, x) = q(z_y|x)q(y|z_y)
\end{align}

\begin{align}
&ELBO(x) 
= E_{q(z_d|x), q(z_x|x), \underbrace{q(z_y, y|x)}_{\text{y is latent now}}}\log p_{\theta}(x|z_d, z_x, z_y) \nonumber\\
&- \beta_x KL(q_{\phi_x}(z_x|x)||p_{\theta_x}(z_x)) - \underbrace{\beta_y E_{q_{\phi_y}(z_y|x)}[\sum_y q(y|z_y) \log\frac{q_{\phi_y}(z_y|x)}{p_{\theta_y}(z_y|y)}]}_{\text{impute y, can not write $\sum_y q(y|z_y)\beta_y KL(q_{\phi_y}(z_y|x)||p_{\theta_y}(z_y|y))$ }} \nonumber \\
&- \underbrace{\beta_d 
E_{q_{\phi_s}(s|x,z_d), q_{\phi_d}(z_d|x)}\log \frac{q_{\phi_d}(z_d|x)}{p_{\theta_d}(z_d|s)}}_{\text{impute $s$: Two layers latent variable, from $y$ to $z_y$ to $x$ and from $s$ to $z_d$ to $x$}} \nonumber\\ &-\beta_sE_{q_{\phi_d}(z_d|x)}KL(q_{\phi_s}(s|z_d)||p_{\theta_s}(s|\alpha)) + \underbrace{-E_{q_{\phi_y}(z_y|x)}\sum_y q(y|z_y)[\log q_{\omega}(y|z_y)-\log p(y)]}_{\text{KL divergence on y, in comparison to $y$ is observed, inversion of sign on $q(y|z_y)$, no $\gamma_y$}}\label{eq:elbo_x}
\end{align}

The double expectation involving $z_y$ can **not** be written as a single expectation: $E_{q(y|z_y)}KL\allowbreak(q(z_y|x)||p((z_y|y)$ since $z_y$ is not observation, the outter most expectation can only take probabilities based on observables like $x$, however, in practice,  the Expectation with respect to $q(z_y|x)$ can be done in a way of Monto Carlo, while expectation with respect to $q(y|z_y)$ is done explicitly by summing up all possible values of $y$. If $y$ is continuous, say, consider $s$ here, we have $\beta_d 
E_{q_{\phi_s}(s|x,z_d), q_{\phi_d}(z_d|x)}\log \frac{q_{\phi_d}(z_d|x)}{p_{\theta_d}(z_d|s)}$, we use a single round Monto Carlo to approximate this expectation, ideally, we should do a double round Monto Carlo. Note this is different for $y$ for example, $-E_{q_{\phi_y}(z_y|x)}\sum_y q(y|z_y)[\log q_{\omega}(y|z_y)-p(y)]$, where an explicit integration with respect to all possible values of $y$ are carried out.

In implementation, the input is a mini-batch of $x$, $E_{q_{\phi_y}(z_y|x)}\sum_y q(y|z_y)[\cdot]$ is done by enumerating all $y$ values for each instance $x$ of the mini-batch, when $y$ has 10 values, it correspond to $10\times M$ terms summation.

\textbf{That being analyzed, we need an approximation to the expectation with respect to $s$ in  $E_{q_{\phi_s}(s|x,z_d), \allowbreak q_{\phi_d}(z_d|x)}[\cdot] = E_{q_{\phi_d}(z_d|x)q_{\phi_s}(s|z_d)}[\cdot]$ or specifically $E_{q_{\phi_s}(s|z_d)}[\cdot]$, the simplest way is to sample $s$ multiple times than just 1 time, conditioned on a sample of $z_d$}


\paragraph{Unsup learn directly from ELBO}
(The following derivation is not complete yet, \ldots)
Since
\begin{align}
q(y|x) = \int_{z_y}q(y,z_y|x)dz_y = \int_{z_y}\frac{q(y,z_y,x)}{q(z_y,x)}\frac{q(z_y,x)}{q(x)}dz_y =\int_{z_y}q(y|z_y)q(z_y|x)dz_y 
\end{align}

so
\begin{align}
  E_{q(y|x)}[\cdot] = \Sigma_y q(y|x)[\cdot]  = \Sigma_y\int_{z_y}q(y|z_y)q(z_y|x)dz_y [\cdot]
\end{align}
In amortized variational inference, the integration is approximated by Monto Carlo samples, only the weight term $q(y|z_y)q(z_y|x)$ remains intact. 

Without class label, the class lable prediction likelihood term $\gamma_y E_{q_{\phi_y}(z_y|x)}[\log q_{\omega}(y|z_y)]$ disappears (does not exist anymore), instead, $y$ as latent variable, its posterior sampled is used to reconstruct the image, its KL divergence need to be added to finish the definition of ELBO of one data point.

\begin{eqnarray}
  ELBO(x) = E_{q(y|x)} \left[ELBO(x,y) - KL\left(q(y|x)||p(y)\right)\right]\label{eq:elbo_plus_y_unsup2}
\end{eqnarray}, where $E_{q_{\omega}(y|z_y)q_{\phi_y}(z_y|x)} ELBO(x,y)$ is difficult to derive.


\subsection{Class semi-supervised learning and supervised learning comparision}
\begin{algorithm}
	\caption{HDIVA} % problem for beamer
        \begin{algorithmic}[1] % the [1] is displaying the line number
		\WHILE{not converged or maximum epochs not reached}
		\STATE warm up $\beta$ defined in Equation \ref{eq:elbo}, as in \cite{sonderby2016ladder}
		\STATE fetch mini-batch \{x, y\} =\{$x^{(l,i)},y^{(l,i)}$\}  \\
		\STATE compute parameters for $q_{\phi_x}(z_x|x)$, $q_{\phi_y}(z_y|x)$, $q_{\phi_d}(z_d|x)$ \\
		\STATE sample latent variable $z_{x}^q$, $z_{y}^q$ and compute $[\log q_{\omega}(y|z_y)]$ in equation \ref{eq:elbo_plus_y}
		\STATE sample $z_d^q$, infer concentration parameter
		$\phi_{s}(z_d)$ and aggregate according to Equation \ref{eq:agg_alpha}
		\STATE sample topic $s$ from aggregated
		 $\phi^{agg}_{s}(z_{d_{1:M}})$ according to Equation \ref{eq:alpha_infer_agg}.
		\STATE compute prior distribution for $z_d$ using $s$
		\STATE adapt posterior of $q_{\phi_d}(z_d)$ with ladder-vae method \cite{sonderby2016ladder}
		\STATE sample $z_{d}^q$ from adapted $q_{\phi_d}(z_d)$ 
		\STATE compute $p_{\theta}(x|z_x,z_y,z_d)$ using sampled $z_{x}^q$, $z_{y}^q$, $z_{d}^q$
		\STATE compute KL divergence for $z_d$, $z_x$ and $z_y$, $s$ in Equation \ref{eq:elbo}
		\STATE compute pair wise MMD of the nominal domains 
		\STATE aggregate loss according to \ref{eq:final} and update model
		\ENDWHILE 
	\end{algorithmic}
	\label{algo:hdiva}
\end{algorithm}


\begin{algorithm}
	\caption{HDIVA-Structured} % problem for beamer
        \begin{algorithmic}[1] % the [1] is displaying the line number
		\WHILE{not converged or maximum epochs not reached}
		\STATE warm up $\beta$ defined in Equation \ref{eq:elbo}, as in \cite{sonderby2016ladder}
		\STATE fetch mini-batch x=\{$x^{(l,i)}$\}  \\
		\STATE compute parameters for $q_{\phi_x}(z_x|x)$, $q_{\phi_y}(z_y|x)$, $q_{\phi_d}(z_d|x)$ \\
		\STATE $x$ path: \\
                sample latent variable $z_{x}^q$ \\
                compute KL divergence for $z_x$ \\
                ; return $z_x$, KL divergence for $z_x$
                \STATE $y$ path (compute KL divergence for $y$ and $z_y$): \\
		sample latent variable $z_{y}^q$ \\
                compute $[\log q_{\omega}(y|z_y)]$ in equation \ref{eq:elbo_plus_y} \\
                ; return $z_y$, KL for y, KL for zy
		\STATE $d$ path: \\
                sample $z_d^q$, infer concentration parameter \\
		$\phi_{s}(z_d)$ and aggregate according to Equation \ref{eq:agg_alpha} \\
		sample topic $s$ from aggregated
		 $\phi^{agg}_{s}(z_{d_{1:M}})$ according to Equation \ref{eq:alpha_infer_agg}.\\
		compute prior distribution for $z_d$ using $s$ \\
		adapt posterior of $q_{\phi_d}(z_d)$ with ladder-vae method \cite{sonderby2016ladder} \\
		sample $z_{d}^q$ from adapted $q_{\phi_d}(z_d)$\\
                ; return $z_d$, KL for $s$, KL for $zd$

		\STATE compute $p_{\theta}(x|z_x,z_y,z_d)$ using sampled $z_{x}^q$, $z_{y}^q$, $z_{d}^q$
		\STATE compute KL divergence for $z_d$, $z_x$ and $z_y$, $s$ in Equation \ref{eq:elbo}
		\STATE compute pair wise MMD of the nominal domains 
		\STATE aggregate loss according to \ref{eq:final} and update model
		\ENDWHILE 
	\end{algorithmic}
	\label{algo:hdiva}
\end{algorithm}


==> t4fig_color_mnist_back.tex <==

\begin{figure}[h!]
	\center\includegraphics[width=0.3\textwidth]{figures/color_mnist_background_only}
	\caption{Color-Mnist-Background}\label{fig:color_mnist_backgrounds}
\end{figure}

==> table_figure_side_by_side.tex <==
\begin{table}[ht]
\begin{minipage}[b]{0.4\linewidth}
\centering
	\includegraphics[width=0.9\textwidth]{source/tikz_ehdiva.pdf}
	%\caption{\textbf{\mname: \fullalgoname}}
\captionof{figure}{\mname:\fullalgoname}
\label{fig:ehdiva}
\end{minipage}\hfill
\begin{minipage}[b]{0.56\linewidth}
\centering
	\caption{ \textbf {Malaria Virtual Hospital from Malaria Dataset}. Patients with ID starting with C1, C6, C8, C9 are grouped to form  4 virtual hospitals as 4 nominal domains.  We report result on the test domain corresponding to virtual hospital C1. 20 repetitions are done where each repetition sub-sample 20 percent of the training domains data as training data and the rest as validation. Comparison algorithms are DIVA \mcitep{ilse2019diva} and Match-DG \mcitep{mahajan2020domain}, while Deep-All is used as baseline by pooling all training domains together. Further detail can be found in supplement \ref{sec:iclr_malaria_supp}.\\Data source: \mcitep{rajaraman2018pre}}
	\begin{tabular}{lc}
		\toprule
		%\multicolumn{4}{|c|}{Style Digit} \\
		%\hline
		\bfseries Malaria Cell Classification  & \bfseries Test Accuracy \\
		\midrule 
		%CVAE     &  0.82, 0.06\\
		DIVA     &  0.83 $\pm$ 0.06\\
		\mname{}    & \textbf{0.87} $\pm$ 0.05 \\
		Deep-All  &  0.84 $\pm$ 0.05 \\
		MatchDG   & 0.85 $\pm$ 0.09 \\
		\bottomrule
	\end{tabular}
	\label{tb:malaria}
\end{minipage}
\end{table}

==> tb_color_combo_rgb_v.tex <==

\begin{table*}[]
    \centering
\begin{tabular}{ |p{3cm}||p{1cm}|p{1cm}|p{1cm}| p{1cm}| p{1cm}|p{1cm}|}
 \hline
 &\multicolumn{3}{|c|}{Foreground} &\multicolumn{3}{|c|}{Background} \\
 \hline
 Subdomain & R & G &B & R & G &B\\
 \hline
 1 &31 & 119 & 180 & 214 & 39 & 40 \\
2 & 255 & 127 & 14 & 44 & 160 & 44 \\
3 & 44 & 160 & 44 & 255 & 127 & 14 \\
4 & 214 & 39 & 40 & 31 & 119 & 180 \\
5 & 148 & 103 & 189 & 23 & 190 & 207 \\
6 & 140 & 86 & 75 & 188 & 189 & 34 \\
7 &227 & 119 & 194 & 127 & 127 & 127 \\
8 &127 & 127 & 127 & 227 & 119 & 194 \\
9 &188 & 189 & 34 & 140 & 86 & 75 \\
10 &23 & 190 & 207 & 148 & 103 & 189 \\
 \hline
\end{tabular}
    \caption{The RGB color for the color combination experiment in section \ref{sec:color-combo}}
    \label{tb:color-combo-rgb-v}
\end{table*}

==> tb_mnist_overlap.tex <==
\begin{table}[h!]
	\centering
	\begin{tabular}{ |p{2cm}||p{2cm}|p{2cm}|}
		\hline
		Test Angle  & DIVA &  HDIVA  \\
		\hline
		0, 22,  75  & 0.821 $\pm$ 0.007    & \textbf{0.9679 $\pm$ 0.003} \\
		\hline
	\end{tabular}\caption{The overlapped Rotated MNIST scenario where the first nominal domain contains rotations of 15, 30, 45 degrees and the second nominal domains contains rotation angles of 30, 45, 60, both algorithms train on two nominal domains and test on out of domain rotation angles at 0, 22, 75 respectively and we report the average accuracy with standard deviation by averaging results from 10 random seeds.}
\label{tb:mnist-overlap}
\end{table}

==> tb_mnist_r.tex <==
\begin{table}[!h]
	\centering
	\renewcommand{\arraystretch}{0.5}
	\begin{threeparttable}
		\caption[Rotated Mnist]{ \textbf{: Rotated Mnist}}
		\begin{tabular*}{0.5\textwidth}{c @{\extracolsep{\fill}} cccccc}
			\toprule
 Test               &  DA   &  LG   &  HEX  &  ADV  &  DIVA      & HDIVA          \\
        	\midrule
 M$_{{0}^{\circ}}$  &  86.7 &  89.7 &  90.1 &  89.9 &  93.5 $\pm{}$ 0.3  &  94.3 $\pm{}$ 0.3   \\
 M$_{{15}^{\circ}}$ &  98.0 &  97.8 &  98.9 &  98.6 &  99.3 $\pm{}$ 0.1 &  99.7 $\pm{}$ 0.1    \\
 M$_{{30}^{\circ}}$ &  97.8 &  98.0 &  98.9 &  98.8 &  99.1 $\pm{}$ 0.1 &  99.6 $\pm{}$ 0.1   \\
 M$_{{45}^{\circ}}$ &  97.4 &  97.1 &  98.8 &  98.7 &  99.2 $\pm{}$ 0.1 &  99.9 $\pm{}$ 0.1    \\
 M$_{{60}^{\circ}}$ &  96.9 &  96.6 &  98.3 &  98.6 &  99.3 $\pm{}$ 0.1 &  99.7 $\pm{}$ 0.1    \\
 M$_{{75}^{\circ}}$ &  89.1 &  92.1 &  90.0 &  90.4 &  93.0 $\pm{}$ 0.4 &  94.0 $\pm{}$ 0.4   \\
           \midrule
% Avg                & 94.3  & 95.3  & 95.8  & 95.2  & 97.2 $\pm{}$ 1.3 & 97.2 $\pm{}$ 1.3    \\  
%	       \bottomrule
		\end{tabular*}
		
		\begin{tablenotes}
			\item  Adapted from \cite{ilse2019diva}
		\end{tablenotes}
		\label{tab:mnistr}
	\end{threeparttable}
\end{table}



==> tb_mnist_rotate.tex <==
\begin{table*}[t]
	\centering
	\begin{tabular}{ |p{3cm}||p{3cm}|p{3cm}|p{3cm}|  }
		\hline
		\multicolumn{4}{|c|}{Mnist Rotation} \\
		\hline
		TestSet  & IFL &  DIVA & HDIVA \\
		\hline
		0 degree   & 0.867    & 0.935 & 0.943\\
		15 degree   & 0.980 & 0.993 &  0.997\\
		30 degree   & 0.978 & 0.991 &  0.996\\
		45 degree   & 0.974  & 0.992 & 0.999\\
		60 degree   & 0.969  & 0.993 & 0.997\\
		75 degree   & 0.891 & 0.930 &  0.940\\
		\hline
	\end{tabular}\caption{Mnist Rotation}
\label{tb:mnistr}
\end{table*}


==> tb_pacs_backup.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\usepackage{geometry}
%\usepackage{array}

%\usepackage{multirow}
%\usepackage{booktabs}
%\usepackage{threeparttablex}
%\usepackage[table]{xcolor}



%\begin{document}

\begin{table*}[t]
	\centering
	\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}
		\caption[Domain Generalization in PACS]{ \textbf{Domain Generalization in PACS}}
		\begin{tabular*}{\textwidth}{c @{\extracolsep{\fill}} cccccc}
			\toprule
			Methods & Venue	      &  Art painting & Cartoon &	Photo & Sketch &  Ave   \\
			\midrule
			      1 &  ICCV'17    &  62.86            &  66.97              &  89.5             &  57.51            &  69.21            \\
                  2 &  AAAI'18    &  66.23            &  66.88              &  88               &  58.96            &  70.01            \\
                  3 &  ICIP'18    &  64.1             &  66.8               &  90.2             &  60.1             &  70.3             \\
                  4 &  NeurIPS'18 &  \textbf{69.82}   &  70.35              &  \textbf{91.07}   &  59.26            &  72.62            \\
                  5 &  ICLR'19    &  66.8             &  69.7               &  87.9             &  \underline{56.3} &  70.2             \\
                  6 &  CVPR'19    &  67.63            &  \textbf{71.71}     &  89               &  \textbf{65.18}   &  \textbf{73.38}   \\
                  7 &  preprint   &  \underline{61.2} &  \underline{63.8}   &  \underline{82.9} &  59               &  \underline{66.7} \\
			\bottomrule
		\end{tabular*}
		
		\begin{tablenotes}
			\item  Adapted from XXXX.
		\end{tablenotes}
		\label{tb:pacs}
	\end{threeparttable}
\end{table*}

%\end{document}


==> tb_pacs_old.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\usepackage{geometry}
%\usepackage{array}

%\usepackage{multirow}
%\usepackage{booktabs}
%\usepackage{threeparttablex}
%\usepackage[table]{xcolor}



%\begin{document}

\begin{table*}[t]
	\centering
	\small
	%\renewcommand{\arraystretch}{1.5}
	\begin{threeparttable}
		\caption[Domain Generalization in PACS Dataset with AlexNet]{\textbf{Domain Generalization in PACS Dataset with AlexNet Classifier}}
		\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} lllll}
			\toprule
			\bfseries Methods 	      & \bfseries Art Painting &  \bfseries Cartoon & \bfseries	Photo & \bfseries Sketch & \bfseries  Ave.   \\
			\midrule
			      Factorization \scriptsize{\mcitep{li2017deeper}}     &  0.63            &  0.67              &  0.90             &  0.58            &  0.69            \\
                  MLDG \scriptsize{\mcitep{li2018learning}}     &  0.66            &  0.67              &  0.88               &  0.59            &  0.70            \\
                  SourceCombo \scriptsize{\mcitep{mancini2018best}}     &  0.64             &  0.67               &  0.90             &  0.60             &  0.70             \\
                  MetaReg \scriptsize{\mcitep{balaji2018metareg}}  &  \textbf{0.70}   &  0.70              &  \textbf{0.91}   &  0.59            &  0.73            \\
                  GLCM \scriptsize{\mcitep{wang2019learning}}     &  0.67             &  0.70               &  0.88             &  0.56 &  0.70             \\
                  Jigsaw \scriptsize{\mcitep{carlucci2019domain}}     &  0.68            &  \textbf{0.72}     &  0.89               &  \textbf{0.65}   &  \textbf{0.74}   \\
                  AFLAC \scriptsize{\mcitep{akuzawa2018domain}}    &  \underline{0.61} &  \underline{0.64}   &  \underline{0.83} &  0.59               &  \underline{0.67} \\
                  
                  MatchDG \scriptsize{\mcitep{mahajan2020domain}}     &0.67 $\pm$0.01 & 0.69 $\pm$ 0.01 &0.89 $\pm$ 0.01 &0.63 $\pm$ 0.02 & 0.72\\
                  %DIVA \cite{ilse2019diva} &  47  & 58    &68    &56 &57.25\\ 
                  %DIVA-AUG      &  50  & 68    & 73   & 43 &58.5 \\
                  %DIVA(elbo)    & 0.66 $\pm$ 0.01   & 0.68 $\pm$ 0.03 &  0.88  & 0.61 0.02 \\
                   DIVA \scriptsize{\mcitep{ilse2019diva}}    & 0.64 $\pm$ 0.02    & 0.66 $\pm$ 0.003 &  0.87 $\pm$ 0.01 & 0.58 $\pm$ 0.03 & 0.69 \\
                    Deep-All & 0.64 $\pm$ 0.01 &  0.67 $\pm$ 0.02 &  0.85 $\pm$ 0.02  &  0.56 $\pm$ 0.02 & 0.68 \\
                  \mname{}  & 0.65 $\pm$ 0.01  & 0.66 $\pm$ 0.01 &  0.87 $\pm$ 0.01  & 0.58 $\pm$ 0.01 & 0.69 \\
                  W\mname{}$^{\ast}$ &  0.64 $\pm$ 0.01  & 0.67 $\pm$ 0.02 & 0.88 $\pm$ 0.01 & 0.60 $\pm$ 0.02 & 0.70\\
                 \mname-no-zx$^{\ast\ast\ast\ast}$ &0.65$\pm$ 0.01 & 0.67$\pm$0.02 & 0.87 $\pm$ 0.01 & 0.61 $\pm$ 0.03 &0.70\\
                 % Sketch(8, 0.6076602, 0.02745811), photo(7, 0.8724675, 0.01425576), cartoon(8, 0.6663462, 0.01720015), art-painting(7, 0.6514706, 0.009921686)
                  L\mname$^{\ast\ast}$ & 0.65 $\pm$ 0.003  & 0.69 $\pm$ 0.02   & 0.87 $\pm$ 0.004 & \underline{0.55 $\pm$ 0.002} & 0.69 \\
                  \mname-CTR$^{\ast\ast\ast}$ & 0.65 $\pm$ 0.01  & 0.66 $\pm$ 0.02   & 0.88 $\pm$ 0.01 &  0.63 $\pm$ 0.003 & 0.71 \\
                  %HDIVA     &  56  & 62    &75   & 56 &62.25 \\
                  %HDIVA-AUG  &54  & 64  &82   & 60 & 65 \\
			\bottomrule
		\end{tabular*}
		
		\begin{tablenotes}
			\item  %Variants of our algorithm in the table:\\
			$^{\ast}$ W\mname: weak domain-supervision added to \mname{} as explained  in Appendix \ref{sec:weak}.\,\,\\ $^{\ast\ast}$L\mname: Ladder \fullalgoname explained in Appendix \ref{sec:lhdiva}.\\
			$^{\ast\ast\ast}$\mname-CTR: Use the contrastive learning phase (pretrain phase) of \mcitet{mahajan2020domain} as initialization for AlexNet of \mname.\\
			$^{\ast\ast\ast\ast}$\mname-no-zx: \mname{} without $z_x$ variable, see Figure~\ref{fig:hduva_no_zx}.\\
			Part of the table is adapted from \url{https://domaingeneralization.github.io/}.
		\end{tablenotes}
		\label{tb:pacs}
	\end{threeparttable}
\end{table*}

%\end{document}


==> tb_pacs_small.tex <==
\begin{table*}[t]
	\begin{tabular}{ |p{3cm}||p{3cm}|p{3cm}|p{3cm}|  }
		\hline
		\multicolumn{4}{|c|}{PACS} \\
		\hline
		TestDomain  & DeepAll(AlexNet) &  DIVA & HDIVA \\
		\hline
		Photo  & 0.60    &   & \\
		Art    & \~0.50 &    & \\
		Sketch & \~0.50 &  \~0.58 & 0.58 \\
		Cartoon & \~0.50 &   &  \\
		\hline
	\end{tabular}
	\caption{PACS dataset}	
	\label{tb:pacs}
\end{table*}

==> tb_semi.tex <==
\begin{table*}[h!]
	\centering
	\begin{tabular}{ |p{3.5cm}||p{3cm}|p{3cm}| p{3cm}| }
		\hline
		Test nominal domains  &  Nominal Domain 1&  Nominal Domain 2 & Nominal Domain 3  \\
		\hline
		HDIVA   &    0.93 $\pm$ 0.02   & 0.845 $\pm$ 0.06  &  0.506 $\pm$ 0.04   \\	HDIVA-Domain-Semi-Sup  & \textbf{0.96}   &\textbf{0.99}  &  \textbf{0.97}   \\
		\hline
	\end{tabular}
	\caption{Domain Label Semi-Supervised Learning of HDIVA: We take another randomly pre-sampled 1000 MNIST instances and color them according to the training sub-domains of Figure \ref{fig:color_mnist_both_combo} but do not give these instances any domain label.}
	\label{tb:semi}
\end{table*}

==> tb_semi_pacs.tex <==
\begin{table*}[h!]
	\centering
        \begin{tabular}{ |p{3.5cm}||p{3cm}|p{3cm}| p{3cm}|p{3cm} }
		\hline
                Test domains  &  ArtPainting & Cartoon & Photo  & Sketch\\
		\hline
                HDIVA &    0.54   & 0.64   &  0.82 & 0.60   \\
		\hline
                HDIVA(80\% train data)   &  0.5123(9729781)   & 0.5966(10043150)  &  0.8072(9821166) & 0.45(10862142)   \\
		\hline
                HDIVA(80\% train data plus 20\% domain unsup)   &0.5167(12651892) & 0.6012(13186077)   &0.7922(12776041)    &0.413 (13203274) \\
		\hline
	\end{tabular}
	\caption{Domain Label Semi-Supervised Learning of HDIVA}
	\label{tb:semi}
\end{table*}


==> tb_style_digit.tex <==
\begin{table*}[t]
	\centering
	\begin{tabular}{ |p{3cm}||p{2cm}|p{2cm}|p{2cm}| p{2cm}| }
		\hline
		%\multicolumn{4}{|c|}{Style Digit} \\
		%\hline
		Methods  & Mnist-M (7,200) &  USPS (5,800) & SVHN (58,600) & Synth (383,520)\\
		\hline
		DIVA     & 0.49   & 0.53 &\textbf{ 0.70}(confirmed) &  \textbf{0.83}\\
		HDIVA-Edge    & 0.50 &  0.52 & 0.54 & 0.76\\
		HDIVA-Flat    & \textbf{0.51} &  \textbf{0.58} &  0.56 &   0.74\\
		\hline
	\end{tabular}
	\caption{Style Digit dataset}
	\label{tb:digit}
\end{table*}




==> tfig_disentangle.tex <==

\begin{figure}[h]
	\center\includegraphics[width=0.3\textwidth]{figures/recon_diva_scan_label_zx_0_zd_q}
	\caption{DIVA Conditional Reconstruction}\label{fig:recon_scan_label_diva}
\end{figure}

\begin{figure}[h]
	\center\includegraphics[width=0.3\textwidth]{figures/recon_hdiva_scan_label_zx_0_zd_q}
	\caption{HDIVA Conditional Reconstruction with (zdq, 0, py)}\label{fig:recon_scan_label_hdiva}
\end{figure}


\begin{figure}[h]
	\center\includegraphics[width=0.3\textwidth]{figures/recon_hdiva_scan_domain_zx_q_zy_q}
	\caption{HDIVA Conditional Reconstruction with (pzd, qzx,qzy)}\label{fig:recon_scan_domain_hdiva}
\end{figure}


\begin{figure}[h!]
	\center\includegraphics[width=0.3\textwidth]{figures/recon_diva_scan_domain_zx_q_zy_q}
	\caption{DIVA Conditional Reconstruction}\label{fig:recon_scan_domain_diva}
\end{figure}


==> to_use_later.tex <==
\begin{figure}[h!]
	\center\includegraphics[width=0.3\textwidth]{figures/dataset}
	\caption{Salad stylized digit}\label{fig:ds_digit_style_salad}
\end{figure}

We propose to use the digit salad \cite{salad}  as in Figure \ref{fig:ds_digit_style_salad} as a benchmark dataset for domain generalization where each dataset comprises a new domain.


\begin{figure}[h!]
	\center\includegraphics[width=0.3\textwidth]{figures/color_mnist_background_only}
	\caption{Color-Mnist-Background}\label{fig:color_mnist_backgrounds}
\end{figure}
